Variational formulations of ODE-Net as a mean-field optimal control problem and existence results

This paper presents a mathematical analysis of ODE-Net, a continuum model of deep neural networks (DNNs). In recent years, Machine Learning researchers have introduced ideas of replacing the deep structure of DNNs with ODEs as a continuum limit. These studies regard the "learning" of ODE-Net as the minimization of a "loss" constrained by a parametric ODE. Although the existence of a minimizer for this minimization problem needs to be assumed, only a few studies have investigated its existence analytically in detail. In the present paper, the existence of a minimizer is discussed based on a formulation of ODE-Net as a measure-theoretic mean-field optimal control problem. The existence result is proved when a neural network, which describes a vector field of ODE-Net, is linear with respect to learnable parameters. The proof employs the measure-theoretic formulation combined with the direct method of Calculus of Variations. Secondly, an idealized minimization problem is proposed to remove the above linearity assumption. Such a problem is inspired by a kinetic regularization associated with the Benamou--Brenier formula and universal approximation theorems for neural networks. The proofs of these existence results use variational methods, differential equations, and mean-field optimal control theory. They will stand for a new analytic way to investigate the learning process of deep neural networks.

==> preamble.tex <==
% \documentclass[leqno,11pt,a4paper]{amsart} %leqno is the option to put formula numbers on the left side
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[hypertexnames=false]{hyperref}
\usepackage[top=28truemm,bottom=28truemm,left=38truemm,right=38truemm]{geometry}
\setlength{\textheight}{23cm}
\setlength{\textwidth}{16cm}
\setlength{\oddsidemargin}{0cm}
\setlength{\evensidemargin}{0cm}
\setlength{\topmargin}{0cm}
\renewcommand{\baselinestretch}{1.1} %changing the interline spacing
\setlength{\parindent}{2em} % 1em = 1quad
\setlength{\parskip}{0.3em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Section title font modified %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \makeatletter
% \renewcommand\section{\@startsection{section}{1}{\z@}%
%           {25\p@ \@plus 6\p@ \@minus 3\p@}%
%           {14\p@ \@plus 6\p@ \@minus 3\p@}%
%           {\fontsize{14pt}{0cm}\selectfont\bfseries\boldmath}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%           {17\p@ \@plus 6\p@ \@minus 3\p@}%
%           {9\p@ \@plus 6\p@ \@minus 3\p@}%
%           {\fontsize{13pt}{0cm}\itshape}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%           {12\p@ \@plus 6\p@ \@minus 3\p@}%
%           {\p@}%
%           {\normalfont\normalsize\itshape}}
% %
% \renewcommand{\paragraph}[1]{%
%   \par% ensure starting on a new paragraph
%   \addvspace{\medskipamount}% some vertical space
%   \noindent
%   \textbf{#1\@addpunct{.}}\enspace\ignorespaces
% }
% \makeatother
\usepackage[TU]{fontenc}
\makeatletter
\renewcommand\section{\@startsection{section}{1}{\z@}%
           {25\p@ \@plus 6\p@ \@minus 3\p@}%
           {10\p@ \@plus 6\p@ \@minus 3\p@}%
           {\fontsize{13pt}{0cm}\selectfont\bfseries\boldmath}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%           {13\p@ \@plus 6\p@ \@minus 3\p@}%
%           {6\p@ \@plus 6\p@ \@minus 3\p@}%
%           {\fontsize{12pt}{0cm}\itshape}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%           {12\p@ \@plus 6\p@ \@minus 3\p@}%
%           {\p@}%
%           {\normalfont\normalsize\itshape}}
           
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
           {13\p@ \@plus 6\p@ \@minus 3\p@}%
           {6\p@ \@plus 6\p@ \@minus 3\p@}%
           {\fontsize{12pt}{0cm}}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
           {12\p@ \@plus 6\p@ \@minus 3\p@}%
           {\p@}%
           {\normalfont\normalsize}}
%
\renewcommand{\paragraph}[1]{%
  \par% ensure starting on a new paragraph
  \addvspace{\medskipamount}% some vertical space
  \noindent
  \textbf{#1\@addpunct{.}}\enspace\ignorespaces
}
\makeatother
% \renewcommand{\thesection}{\bf{\arabic{section}}}
% \renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}
% \renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Table of contents modified %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{tocdepth}{1}% to get subsubsections in toc
\let\oldtocsection=\tocsection
\let\oldtocsubsection=\tocsubsection
\let\oldtocsubsubsection=\tocsubsubsection
\renewcommand{\tocsection}[2]{%\\  \noindent
\hspace{0em}\bfseries\oldtocsection{#1}{#2}}
\renewcommand{\tocsubsection}[2]{\hspace{1em}\small\oldtocsubsection{#1}{#2}}
\renewcommand{\tocsubsubsection}[2]{\hspace{2em}\small\oldtocsubsubsection{#1}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
% \bibliographystyle{junsrt}
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,hypertexnames=false]{hyperref}
\usepackage[dvipdfmx,x11names,dvipsnames]{xcolor}
\usepackage[dvipdfmx]{graphicx}
\usepackage{url}
% biblatex
\usepackage[doi=false,isbn=false, sortcites=true,eprint=true, date=year, style=numeric,uniquename=init,giveninits=true,sorting=nty,url=false,maxnames=99,backref=true]{biblatex} % alphabetic
% \usepackage[backend=biber]{biblatex}
% \usepackage[doi=false,isbn=false, sortcites=true,eprint=true, date=year, style=authoryear,uniquename=init,giveninits=false,sorting=none,url=false,maxnames=99]{biblatex} % author year

% How to get BibLaTeX-chicago use title case capitalization?
% https://tex.stackexchange.com/questions/97698/how-to-get-biblatex-chicago-use-title-case-capitalization
\usepackage{filecontents}


\DeclareFieldFormat*{volume}{\mkbibbold{#1}} 
\DeclareFieldFormat*{title}{\mkbibquote{#1\adddot}}  
\DeclareFieldFormat*{booktitle}{\mkbibemph{#1}}  
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map{
      \step[fieldsource=edition,
            match=\regexp{^(\d+)\.\s+(ed.|edition)$},
            replace=\regexp{$1}]
    }
  }
}
\DeclareFieldFormat*{journaltitle}{\mkbibemph{#1}} 
\DeclareFieldFormat[article,Article,book,inbook,incollection,inproceedings,patent,thesis,unpublished,misc]{year}{#1} %
\renewbibmacro{in:}{} %
\renewbibmacro*{issue+date}{%
  \printfield{issue}%
  \setunit*{\addspace}%
  \usebibmacro{date}%
  \newunit} %
\addbibresource{reference.bib}


% \usepackage[dvipdfmx,hypertexnames=false
% ]{hyperref}
\hypersetup{
    colorlinks=true,
    citecolor=blue,
    linkcolor=blue,
    urlcolor=teal,
    breaklinks=true
}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage[capitalize,noabbrev,nameinlink]{cleveref}
\newcommand{\creflastconjunction}{, and\nobreakspace}
\usepackage{amsthm}
% \usepackage{showkeys} 
%%%%%%%%%%%%%%%%% proof environment %%%%%%%%%%%%%%%%
\expandafter\let\expandafter\oldproof\csname\string\proof\endcsname
\let\oldendproof\endproof
\renewenvironment{proof}[1][\proofname]{%
  \oldproof[\bfseries\itshape #1] 
}{\oldendproof}
% 
\makeatletter
\newenvironment{stop_proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item\relax
  {\itshape\bfseries \IfValueTF{#1}{Proof of #1}{Proof}.}
  % {\itshape Proof of
  % #1\@addpunct{.}}
  \hspace\labelsep\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
\makeatother
% \makeatletter
% \renewenvironment{proof}[1][\proofname]{\par
%   \pushQED{\qed}%
%   \normalfont \topsep6\p@\@plus6\p@\relax
%   \trivlist
%   \item\relax
%   {\itshape\bfseries \IfValueTF{#1}{Proof of #1}{Proof}.}\hspace\labelsep\ignorespaces
% }{%
%   \popQED\endtrivlist\@endpefalse
% }
% \makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\qedsymbol{$\blacksquare$}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{achievement}{Achievement}
\renewcommand\theachievement{\Roman{achievement}}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
% \newtheorem{corollary}[theorem]{Corollary}

\usepackage{array}
\usepackage{latexsym}
\usepackage{subfiles}
\usepackage{amsmath}
\usepackage{optidef}
\allowdisplaybreaks[4]
\usepackage{stackengine}
\usepackage{empheq}

\usepackage{here}
\usepackage{longtable}
\usepackage{lipsum}
\usepackage{subcaption}
\usepackage{caption}
\usepackage{capt-of}
\usepackage{threeparttable}
% \usepackage{stix2}
% \usepackage[upint]{stix}
% \usepackage{newtxtext}
% \usepackage{newtxmath}
\usepackage{upgreek}
\usepackage{boldline}
\usepackage{multirow}
\usepackage{here}
\usepackage[super]{nth}
\usepackage{svg}
\usepackage{enumitem}
\setlist[description]{%
  topsep=10pt,               % space before start / after end of list
  itemsep=5pt,               % space between items
  font={\bfseries\rmfamily}, % set the label font
%  font={\bfseries\sffamily\color{red}}, % if colour is needed
}
\newlist{myenum}{enumerate}{3}
\setlist[myenum,1]{label=\textbf{\arabic*.},
                   ref  =\textbf{\arabic*.}}
\setlist[myenum,2]{label=\textbf{(\alph*)},
                   ref  =\themyenumi\textbf{(\alph*)}}
\setlist[myenum,3]{label=\bfseries(\roman*),
                   ref  =\themyenumii\textbf{.(\roman*)}}


%%%%%%%%%%%%%%||||||&&&&&&&&&&&&&&&&&&&
\usepackage{mathtools}
\usepackage{etoolbox}
\usepackage{breqn}
\usepackage{physics}
\renewcommand*{\eval}[1]{\left.{#1}\right|}

\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
<-6> matha5 <6-7> matha6 <7-8> matha7
<8-9> matha8 <9-10> matha9
<10-12> matha10 <12-> matha12
}{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}

\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
<-6> mathx5 <6-7> mathx6 <7-8> mathx7
<8-9> mathx8 <9-10> mathx9
<10-12> mathx10 <12-> mathx12
}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

\DeclareMathDelimiter{\vvvert} {0}{matha}{"7E}{mathx}{"17}%

\DeclarePairedDelimiterX{\normiii}[1]
{\vvvert}
{\vvvert}
{\ifblank{#1}{\:\cdot\:}{#1}}
\usepackage{appendix}

%%%%%%%%%%%%%%%Englsh font %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% fonts %%%%%%%%%%%%%%%%%%%%%
\SetMathAlphabet{\mathcal}{normal}{OMS}{cmsy}{m}{n} % fixes ugly \mathcals
\SetMathAlphabet{\mathcal}{bold}{OMS}{cmsy}{m}{n} % fixes ugly \mathcals
% \usepackage{charter} % uses normal math fonts this way
% \usepackage{helvet}
% \usepackage[upint]{stix}
%\usepackage{arev}
\DeclareSymbolFont{EulerExtension}{U}{euex}{m}{n}
\DeclareMathSymbol{\euintop}{\mathop} {EulerExtension}{"52}
\DeclareMathSymbol{\euointop}{\mathop} {EulerExtension}{"48}
\let\intop\euintop
\let\ointop\euointop
\DeclareSymbolFont{cmletters}{OML}{cmm}{m}{it}
\DeclareSymbolFont{cmsymbols}{OMS}{cmsy}{m}{n}
\DeclareSymbolFont{cmlargesymbols}{OMX}{cmex}{m}{n}
\DeclareMathSymbol{\myjmath}{\mathord}{cmletters}{"7C}
\DeclareMathSymbol{\myamalg}{\mathbin}{cmsymbols}{"71}
\DeclareMathSymbol{\mycoprod}{\mathop}{cmlargesymbols}{"60}
\let\jmath\myjmath
\let\amalg\myamalg
\let\coprod\mycoprod
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\numberwithin{equation}{section}
% \renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\labelenumi}{\rm (\roman{enumi})}
\allowdisplaybreaks[4]

%%%%%%%%%% tikz %%%%%%%%%%
\usepackage{makecell}
\usepackage{tikz}
\usetikzlibrary{calc}
%% https://tex.stackexchange.com/questions/55068/is-there-a-tikz-equivalent-to-the-pstricks-ncbar-command
\tikzset{
    ncbar angle/.initial=90,
    ncbar/.style={
        to path=(\tikztostart)
        -- ($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)
        -- ($(\tikztotarget)!($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztostart)$)
        -- (\tikztotarget)
    },
    ncbar/.default=0.5cm,
}

\tikzset{square left brace/.style={ncbar=0.5cm}}
\tikzset{square right brace/.style={ncbar=-0.5cm}}

\tikzset{round left paren/.style={ncbar=0.5cm,out=120,in=-120}}
\tikzset{round right paren/.style={ncbar=0.5cm,out=60,in=-60}}
\usetikzlibrary{positioning, fit}   
\tikzset{block/.style={draw, thick, text width=2cm ,minimum height=1.3cm, align=center},   
line/.style={-latex}     
}  


\crefname{theorem}{Theorem}{Theorems}
\crefname{definition}{Definition}{Definitions}
\crefname{problem}{Problem}{Problems}
\crefname{fact}{Fact}{Facts}
\crefname{proposition}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corolary}{Corolary}{Corolaries}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{claim}{Claim}{Claims}

\crefname{remark}{Remark}{Remarks}
\crefname{example}{Example}{Examples}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{subsubsection}{Subsubsection}{Subsubsections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{section}{Section}{Sections}
\crefname{chapter}{Chapter}{Chapters}
\crefname{table}{Table}{Tables}
\crefname{figure}{Figure}{Figures}
\crefname{algorithm}{Algorithm}{Algorithms}
% \crefname{subfigure}{Figure}{Figures}

\crefname{myenumi}{item}{items}
\crefname{myenumii}{item}{items}
\crefname{myenumiii}{item}{items}

\let\normalref\ref
\renewcommand{\ref}{\cref}

% some technical command
% \DeclareSymbolFont{uplargesymbols}{OMX}{mdbch}{m}{n}
% \DeclareMathSymbol{\upintop}{\mathop}{uplargesymbols}{82}
% \newcommand{\upint}{\upintop\nolimits}
\newcommand{\e}{\mathrm{e}}
% \newcommand{\Pc}{\mathcal{P
\newcommand{\Pc}{\mathcal{P}_\mathrm{c}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Ptwo}{\Pcal_2}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Ccinf}{C_c^\infty}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\XtimesY}{\X\times\Y}
\newcommand{\metricsp}{\mathcal{M}}
\newcommand{\Hilbertsp}{\mathcal{H}}
\newcommand{\AC}{\mathrm{AC}}
\newcommand{\Ltwotheta}{L^2\qty(0,1;\mathcal{P}_2(\R^m))}
\newcommand{\varThetaSpace}{L^2\qty(0,1;L^2\qty(\Omega;\R^m))}
\newcommand{\varThetaBochner}{L^2\qty(\qty[0,1]\times\Omega;\R^m)}
\newcommand{\tildeE}{\widetilde{E}}
\newcommand{\OptPlan}{\Gamma_{\mathrm{o}}}
\newcommand{\hatt}{\widehat{t}}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\intRd}{\int_{\R^d}}
\newcommand{\linearization}{\mathcal{L}_\varTheta}
\newcommand{\intRdY}{\int_{\R^d\times\Y}}
\newcommand{\weakast}{\mathrel{\ensurestackMath{\stackon[1pt]{\rightharpoonup}{\scriptstyle\ast}}}}
\newcommand{\doublehookrightarrow}{%
    \mathrel{\mathrlap{{\mspace{4mu}\lhook}}{\hookrightarrow}}
}
\newcommand{\one}{\mathrm{I}}
\newcommand{\two}{\one\hspace{-1.2pt}\one}
\newcommand{\three}{\one\hspace{-1.2pt}\one\hspace{-1.2pt}\one}
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother
\DeclareMathOperator{\Div}{\mathrm{div}}
\DeclareMathOperator{\Ker}{\mathrm{Ker}}
\DeclareMathOperator{\Law}{\mathrm{Law}}
\DeclareMathOperator{\Expect}{\mathbb{E}}
\DeclareMathOperator{\Ldiff}{\mathrm{D}}
\DeclareMathOperator*{\argmax}{\mathop{\rm arg~max}}
\DeclareMathOperator*{\argmin}{\mathop{\rm arg~min}}
\DeclareMathOperator*{\Lip}{\mathrm{Lip}}
\DeclareMathOperator*{\supp}{\mathrm{supp}}
\DeclareMathOperator*{\minimize}{\mathrm{minimize}}
\DeclareMathOperator*{\diam}{\mathrm{diam}}
\DeclareMathOperator{\Hessian}{\mathrm{Hess}}
\DeclareMathOperator*{\Span}{\mathrm{Span}}
\DeclareMathOperator{\ReLU}{\mathrm{ReLU}}
\DeclareMathOperator{\vol}{\mathrm{vol}}
\DeclareMathOperator{\Id}{\mathrm{Id}}
\DeclareMathOperator{\rightexp}{\overrightarrow{\exp}}
\DeclareMathOperator{\Tan}{\mathrm{Tan}}
\DeclareMathOperator*{\Tracee}{\mathrm{Tr}}
\DeclareRobustCommand{\stirling}{\genfrac\{\}{0pt}{}}
\def\Set#1{\Setdef#1\Setdef}
\def\Setdef#1|#2\Setdef{\left\{#1\,\;\mathstrut\vrule\,\;#2\right\}}%
\let\thorn\th % so that thorn-rune \th is not lost
\renewcommand{\th}{%
    \ifmmode% math mode
        ^\mathrm{th}%
    \else%
        \textsuperscript{th}\xspace%
    \fi%
}
\makeatletter
\newcommand{\subalign}[1]{%
  \vcenter{%
    \Let@ \restore@math@cr \default@tag
    \baselineskip\fontdimen10 \scriptfont\tw@
    \advance\baselineskip\fontdimen12 \scriptfont\tw@
    \lineskip\thr@@\fontdimen8 \scriptfont\thr@@
    \lineskiplimit\lineskip
    \ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\hfil\crcr
      #1\crcr
    }%
  }%
}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

